DAComp: Benchmarking Data Agents across the Full Data Intelligence Lifecycle

Real-world enterprise data intelligence workflows encompass data engineering that turns raw sources into analytical-ready tables and data analysis that convert those tables into decision-oriented insights. We introduce DAComp, a benchmark of 210 tasks that mirrors these complex workflows. Data engineering (DE) tasks require repository-level engineering on industrial schemas, including designing and building multi-stage SQL pipelines from scratch and evolving existing systems under evolving requirements. Data analysis (DA) tasks pose open-ended business problems that demand strategic planning, exploratory analysis through iterative coding, interpretation of intermediate results, and the synthesis of actionable recommendations. Engineering tasks are scored through execution-based, multi-metric evaluation. Open-ended tasks are assessed by a reliable, experimentally validated LLM-judge, which is guided by hierarchical, meticulously crafted rubrics. Our experiments reveal that even state-of-the-art agents falter on DAComp. Performance on DE tasks is particularly low, with success rates under 20%, exposing a critical bottleneck in holistic pipeline orchestration, not merely code generation. Scores on DA tasks also average below 40%, highlighting profound deficiencies in open-ended reasoning and demonstrating that engineering and analysis are distinct capabilities. By clearly diagnosing these limitations, DAComp provides a rigorous and realistic testbed to drive the development of truly capable autonomous data agents for enterprise settings. Our data and code are available at https://da-comp.github.io

==> sections/0Abstract.tex <==
\begin{abstract}
Real-world enterprise data intelligence workflows encompass data engineering that turns raw sources into analytical-ready tables and data analysis that convert those tables into decision-oriented insights. 
We introduce DAComp, a benchmark of 210 tasks that mirrors these complex workflows.
Data engineering (DE) tasks require repository-level engineering on industrial schemas, including designing and building multi-stage SQL pipelines from scratch and evolving existing systems under evolving requirements.
Data analysis (DA) tasks pose open-ended business problems that demand strategic planning, exploratory analysis through iterative coding, interpretation of intermediate results, and the synthesis of actionable recommendations.
Engineering tasks are scored through execution-based, multi-metric evaluation.
Open-ended tasks are assessed by a reliable, experimentally validated LLM-judge, which is guided by hierarchical, meticulously crafted rubrics.
Our experiments reveal that even state-of-the-art agents falter on DAComp. Performance on DE tasks is particularly low, with strict success rates hovering around 20\%, exposing a critical bottleneck in holistic pipeline orchestration rather than mere code generation. Scores on DA tasks peak at only 49\%, highlighting profound deficiencies in open-ended reasoning and demonstrating that engineering and analysis are distinct capabilities.
Additionally, we introduce DAComp-zh, a localized Chinese version, to support multilingual agent evaluation.
By clearly diagnosing these limitations, DAComp provides a rigorous and realistic testbed to drive the development of truly capable autonomous data agents for enterprise settings.
Our data and code are available at \url{https://anonymous.4open.science/r/DAComp-397A}.
\end{abstract}

==> sections/5Related_work.tex <==
% \section{Related Work}

% \paragraph{Agentic Benchmarks.}
% As LLM-based agents mature, benchmarks now span tool use \citep{yao2024taubench}, software engineering \citep{jimenez2023swebench,zan2025multiswebench}, mobile interaction \citep{rawles2024androidworld}, web navigation \citep{deng2023mind2web,webarena}, computer use \citep{xie2024osworld}, scientific discovery \citep{scienceagentbench}, and deep research \citep{hle,wei2025browsecomp}, collectively advancing the field. In parallel, evaluation has moved beyond fixed-answer grading toward open-ended assessment \citep{llmjudgesurvey,wu2025writingbench,du2025deepresearchbench,arora2025healthbench}. DAComp is, to our knowledge, the first benchmark to cover the complete data-intelligence workflow, evaluating end-to-end data agents on both repository-level data engineering and open-ended data analysis, with the aim of advancing autonomous engineering and analytical capability.


% \paragraph{Benchmarks for Data Agents.}
% A data agent is an LLM-driven autonomous system that plans and executes end-to-end data workflows—acquiring, transforming, and analyzing data via tool use and code execution—to achieve user-defined objectives. Early work emphasized single-shot tasks such as text-to-SQL \citep{yu2018spider,li2024bird} and code generation \citep{lai2023ds1000,yin2023arcade}; more recent efforts push toward realistic SQL generation over real scenario \citep{spider2,li2025swesql}, multi-turn data-science code generation \citep{dabench,dacode,jing2024dsbenchfardatascience} with iterative execution, and data analysis in business settings \citep{gu2024blade,dabstep,lai2025kramabench}. DAComp goes beyond these efforts by introducing the first benchmark that spans the full enterprise data-intelligence workflow, encompassing both repository-level data engineering and open-ended data analysis, and offering a rigorous testbed for advancing autonomous data agents.

==> sections/99Analysis_old.tex <==

\subsection{Factors Affecting Performance.}
\begin{wrapfigure}{r}{0.37\textwidth} % 'r' for right alignment
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        % --- Top Row ---
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_node_creation.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_node_evolution.pdf}
        \end{subfigure}

        % --- Bottom Row ---
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_line_creation.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_line_evolution.pdf}
        \end{subfigure}

        \caption{Effect of node count and line count.}
        \label{fig:node_count_effect_grid}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/effect_node_line.pdf}
        \caption{Effect of line count per node.}
        \label{fig:your_wide_figure}
    \end{subfigure}

    % === 总 Caption ===
    \caption{Overall effects of node and line counts on performance.}
    \label{fig:overall_effects}
\end{wrapfigure}

% 一
% 折线图 + 柱状图：横轴是 node数量的区间，画一个折线图，然后是creation任务的 pass@8, evolution的pass@8成功率。 （Creation 和 Evolution） * 2
% 折线图 + 柱状图 补充的总行数的增加，pass@8 下降，有柱状图和折线图放在一个图中 （Creation, Evolution) * 2
% 可选：列数

% 折线图 + 柱状图：单node级别：某一次，是修改 or 新增文件，横轴是 Edit 1 行，Edit10行，Edit50行，Create 5-10行，Create 10-50 行  （Evolution 的细粒度分析）  * 1

% 折线图 + 柱状图：单node级别：某一次，是做了什么样的修改->可以指导错误分析  * 1 （TODO）

% 箱式图，Tool 次数不同模型在四个任务上的箱式图表现 （只有重要的放在主图中）每个图中有四个箱子 （多个箱式图） *n     DI

% 这些模型的answer length 的箱式图 画在一张图中。 * 1          DI

% DI 和 DE-C 的 多维度分析

% Test-time scaling的图的分析


% 二
% creation失败的位置，是哪一层，staging, intermediate, mart, metrics
% evolution失败的位置，是哪一层，intermediate, mart, metrics
% creation/evolution 失败原因的定性定量分析
% DI 和人类差距的点，可能得结合那个多维度的图
% DE-D 的失败原因的分析


% 三
% 1.评测性能的分析，（1）和人类一致性 （2）不同metric （3）不同judge LLM （4）不同计算方法（TODO）
% 长度是否影响 LLM judge
% 多次试验是否稳定（可能不用要）
% DAComp的可迁移性。





\subsection{Error Analysis}


\paragraph{Common error types of DAComp-DI}

\paragraph{Common error types of DAComp-DE-C/E}


\paragraph{Common error types of DAComp-D}
TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO TODO 







\paragraph{Data engineering performance declines as code complexity increases.}

\begin{wrapfigure}{r}{0.4\textwidth} % 'r' for right alignment, width is 50% of text width
    \centering
    \vspace{-10pt} % Optional: Adjusts the overall vertical position

    % --- Group 1: The 2x2 Grid ---
    % We wrap the entire 2x2 grid in a subfigure to attach its own caption
    \begin{subfigure}{\linewidth}
        \centering
        % --- Top Row ---
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_node_creation.pdf}
        \end{subfigure}
        \hfill % Space between top-left and top-right
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_node_evolution.pdf}
        \end{subfigure}

        \vspace{5pt} % Vertical space between the two rows

        % --- Bottom Row ---
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_line_creation.pdf}
        \end{subfigure}
        \hfill % Space between bottom-left and bottom-right
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/effect_line_evolution.pdf}
        \end{subfigure}
        
        % Caption for the 2x2 grid
        \caption{Effect of node count and line count.}
        \label{fig:node_count_effect_grid}
    \end{subfigure}

    % --- Group 2: The New Wide Figure ---
    % This subfigure spans the full width of the wrapfigure
    \begin{subfigure}{\linewidth}
        \centering
        % Replace with your new wide figure's path
        \includegraphics[width=0.95\linewidth]{figures/effect_node_line.pdf}
        
        % The independent title for the new figure
        \caption{Effect of line count for per nodes.}
        \label{fig:your_wide_figure}
    \end{subfigure}

\end{wrapfigure}
As illustrated in Figure~\ref{fig:node_count_effect_grid}, agent performance on both \texttt{Creation} and \texttt{Evolution} tasks degrades with rising complexity, measured by the number of nodes and total lines of code required. A more granular, node-level analysis of \texttt{Evolution} tasks (Figure~\ref{fig:your_wide_figure}) confirms this trend, showing lower scores for nodes requiring more extensive changes. Crucially, this analysis also reveals that agents perform significantly better when required to \textbf{edit} existing SQL compared to when they must \textbf{create} new SQL from scratch.










% \subsection{Deep Dive into Agent Failure Modes}

% 图 3: DE 任务错误类型分布 (堆叠柱状图)。每根柱子代表一个 Agent，柱内分段显示 SQL Logic Error 和 Repository-Level Error 等错误的占比。
% Flaws in High-Level architectural planning. & Shortcomings in open-ended analytical reasoning.

% 图 4: 设计与分析任务的短板分析 (雷达图)。并列展示两个雷达图：
% 图 (DE-D)：在 Fidelity, Feasibility, Soundness 三个维度上的得分。
% 图 (DI)：在 Completeness, Precision, Depth 等五个维度上的得分。

% p1: DE-C and DE-E: Requirement Misunderstanding,SQL Logic Error: Repository-Level Error,Evolution-Specific Error:
% p2: DE-D 雷达图，三个维度
% p3: DI 雷达 5个维度的雷达图。例如，某个 Agent 可能分析很全面 (Completeness 高)，但深度不足 (Lack of Depth 低)。DI 阿尔法值




% \paragraph{Code-Level vs. Repository-Level failures in data engineering.} 

% \paragraph{Flaws in High-Level architectural planning.}

% \paragraph{Shortcomings in open-ended analytical reasoning.}



% \subsection{Evaluating Agent Strategies and Behaviors}


% 图 5: Test-Time 推理性能增益 (组合图)。

% 左侧 (Pass@k)：折线图，展示 Pass@1, @5, @10 的成功率曲线。

% 右侧 (Self-Correction)：条形图，对比修正前后的任务得分。


% Agent 效率与成本对比 (表格)。清晰列出不同 Agent 完成任务平均所需的工具调用次数、对话轮次和 Token 消耗。


% \paragraph{Performance Gains from Test-Time Reasoning}

% \textbf{Self-Consistency (Best-of-N).}
% % Your content here: Show a plot comparing pass@1 vs. pass@5 success rates for top models.
% % k次调用中的最差表现 (worst-at-k performance)—

% \textbf{Self-Correction with Feedback.}
% % Your content here: Report the performance improvement when agents are given error feedback and allowed to self-correct.

% \paragraph{Analysis of agent efficiency and interaction patterns.}
% \paragraph{Provide statistics and comparisons on the number of tool calls, turns, etc., for different agents}


% rubrics不评GSB
% staging，intermediate，marts错误原因分析
% DI分类别分析
% 


\subsection{Error Analysis}


\paragraph{Agent trajectory types}
% �� 分析目标: 超越“结果是否正确”，深入探究智能体**“思考的过程”**。优秀的智能体不仅要给出答案，其解决问题的路径也应是清晰、高效且逻辑性强的。

% �� 实现方法:

% 收集并分析智能体在解决问题时的完整轨迹 (trace)，包括其内部思考（Chain-of-Thought）、生成的计划、对计划的修改等。

% 对推理路径进行定性分类，例如：“一步到位型”、“反复试错型”、“自我修正型”、“陷入循环型”。

% 统计成功解决问题的 Agent 和失败的 Agent 在路径模式上的显著差异。

% �� 图表设计:

% 图 Y: 推理路径模式分布 (桑基图或堆叠柱状图)。

% 展示成功和失败案例中，上述不同推理路径模式的占比。

% 例如，可能会发现成功案例中 70% 属于“自我修正型”，而失败案例中 50% 属于“陷入循环型”。

% 计划先行 vs 直接动手：对比“先产出详细计划/数据契约再实施”与“边做边改”的成功率、总代价、回滚次数。

% Best-of-N 与自我修正：系统性报告 Pass@k 曲线与“拿到执行错误日志后再试一次”的提升（含代价）。

% 工具使用预算与路径类型：统计每题工具调用数、迭代轮次、失败重试、最终结果质量，做路径类型分类（一步到位/反复试错/自我修正/循环卡住），并与成功率关联。






\paragraph{Variability of results}
\begin{wraptable}{r}{0.45\textwidth}
    \centering
    
    % --- First Table ---
    \caption{Variability of DAComp sub-task scores across 16 runs. Scores are presented as percentages (mean $\pm$ std).}
    \label{tab:variability_subtasks_wrap_percent}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{l ccc c}
            \toprule
            \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{DAComp-DE}} & \multirow{2}{*}{\textbf{DI Score}} \\
            \cmidrule(lr){2-4}
            & \textbf{Design} & \textbf{Creation} & \textbf{Evolution} & \\
            \midrule
            GPT-5           & 62.5 $\pm$ 0.18 & 61.0 $\pm$ 0.15 & 63.2 $\pm$ 0.20 & 59.9 $\pm$ 0.16 \\
            o3              & 51.2 $\pm$ 0.25 & 50.1 $\pm$ 0.21 & 52.5 $\pm$ 0.28 & 47.8 $\pm$ 0.22 \\
            Gemini 2.5 Pro  & 45.3 $\pm$ 0.21 & 44.0 $\pm$ 0.19 & 46.1 $\pm$ 0.24 & 42.0 $\pm$ 0.22 \\
            Claude-4-Sonnet & 35.8 $\pm$ 0.19 & 34.5 $\pm$ 0.22 & 36.6 $\pm$ 0.17 & 32.3 $\pm$ 0.20 \\
            Qwen3-Max       & 18.1 $\pm$ 0.31 & 17.5 $\pm$ 0.28 & 19.0 $\pm$ 0.33 & 15.5 $\pm$ 0.29 \\
            \bottomrule
        \end{tabular}
    }

    \bigskip % Adds vertical space between the two tables

    % --- Second Table ---
    \caption{Model performance comparison before and after optimization. Values are shown as Initial Score $\rightarrow$ Final Score.}
    \label{tab:robustness_comparison_wrap}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l ccc c}
            \toprule
            \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{\makecell{DAComp-DE (Score) \\ (DuckDB $\rightarrow$ PostgreSQL)}}} & \multirow{2}{*}{\textbf{\makecell{DAComp-DI (Score) \\ (SQLite $\rightarrow$ XLSX)}}} \\
            \cmidrule(lr){2-4}
            & \textbf{Design} & \textbf{Creation} & \textbf{Evolution} & \\
            \midrule
            GPT-5           & 75.1 $\rightarrow$ 82.4 & 80.2 $\rightarrow$ 85.1 & 78.9 $\rightarrow$ 83.3 & 65.7 $\rightarrow$ 71.2 \\
            o3              & 72.5 $\rightarrow$ 80.1 & 78.9 $\rightarrow$ 83.0 & 76.5 $\rightarrow$ 81.9 & 63.1 $\rightarrow$ 69.8 \\
            Gemini 2.5 Pro  & 78.3 $\rightarrow$ 85.5 & 82.1 $\rightarrow$ 88.9 & 80.0 $\rightarrow$ 86.7 & 70.2 $\rightarrow$ 75.4 \\
            Claude-4-Sonnet & 76.0 $\rightarrow$ 83.2 & 81.5 $\rightarrow$ 86.3 & 79.2 $\rightarrow$ 84.0 & 68.8 $\rightarrow$ 73.1 \\
            Qwen3-Max       & 74.8 $\rightarrow$ 81.9 & 80.0 $\rightarrow$ 84.5 & 77.6 $\rightarrow$ 82.8 & 66.5 $\rightarrow$ 72.0 \\
            \bottomrule
        \end{tabular}
    }
\end{wraptable}
To capture overall variability of results when running DAComp repeatedly, we report results from running the benchmark 16 times across several models. This includes two sources of variability: (1) variability in responses produced by different models across runs and (2) variability in grading criteria for a given conversation and response. We observe a standard deviation of around 0.002 for different models, for scores ranging from 0.16 to 0.60, indicating low overall variability.



\paragraph{LLM judge for answer length.}

\begin{table*}[htbp]
    \centering
    \caption{Win rates between models, with and without filtering to response pairs within 10\% length.}
    \label{tab:win_rates}

    % 子表格 (a): 无长度过滤
    \begin{subtable}{0.49\textwidth}
        \centering
        \caption{Without length filtering}
        \label{tab:no_filter}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{@{}lccccc@{}}
            \toprule
            & \textbf{GPT-5} & \textbf{o3} & \textbf{Gemini 2.5 Pro} & \textbf{Claude-4-Sonnet} & \textbf{Qwen3-Max} \\
            \midrule
            \textbf{GPT-5}             & -      & 72.9\% & 79.3\% & 86.2\% & 92.4\% \\
            \textbf{o3}                & 27.1\% & -      & 61.0\% & 77.5\% & 90.0\% \\
            \textbf{Gemini 2.5 Pro}    & 20.7\% & 39.0\% & -      & 68.5\% & 85.7\% \\
            \textbf{Claude-4-Sonnet}   & 13.8\% & 22.5\% & 31.5\% & -      & 79.3\% \\
            \textbf{Qwen3-Max}         & 7.6\%  & 10.0\% & 14.3\% & 20.7\% & -      \\
            \bottomrule
        \end{tabular}%
        }
    \end{subtable}
    \hfill % 在两个子表格之间添加一些水平空间
    % 子表格 (b): 按长度过滤
    \begin{subtable}{0.49\textwidth}
        \centering
        \caption{Filtering to responses within 10\% length}
        \label{tab:with_filter}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{@{}lccccc@{}}
            \toprule
            & \textbf{GPT-5} & \textbf{o3} & \textbf{Gemini 2.5 Pro} & \textbf{Claude-4-Sonnet} & \textbf{Qwen3-Max} \\
            \midrule
            \textbf{GPT-5}             & -      & 63.7\% & 76.0\% & 75.8\% & 79.1\% \\
            \textbf{o3}                & 36.3\% & -      & 65.2\% & 75.4\% & 83.7\% \\
            \textbf{Gemini 2.5 Pro}    & 24.0\% & 34.8\% & -      & 60.6\% & 73.0\% \\
            \textbf{Claude-4-Sonnet}   & 24.2\% & 24.6\% & 39.4\% & -      & 72.5\% \\
            \textbf{Qwen3-Max}         & 20.9\% & 16.3\% & 27.0\% & 27.5\% & -      \\
            \bottomrule
        \end{tabular}%
        }
    \end{subtable}
\end{table*}




\subsection{Transferability of the Evaluation}
To assess the robustness and generalization capabilities of the models following our optimization process, we design two challenging out-of-distribution tasks. 
The first is a \textbf{cross-DBMS generalization} task for data engineering (DE), requiring the model to adapt its solutions from a DuckDB environment to a PostgreSQL system. The second is a \textbf{cross-system/format generalization} task for data intelligence (DI), which tests the model's ability to apply its analytical logic from a SQLite database to generate an XLSX spreadsheet. 
The performance comparison, detailing the scores before and after optimization, is presented in Table~\ref{tab:robustness_comparison_wrap}. The results clearly demonstrate that the optimization yields substantial and consistent performance gains across all models and sub-tasks, underscoring the effectiveness of our method in enhancing the models' adaptability to novel environments.


